92c/MFlops/s, Ultra-Large-Scale Neural-Network Training on a PIII Cluster

Artificial neural networks with millions of adjustable parameters and a similar number of training examples are a potential solution for difficult, large-scale pattern recognition problems in areas such as speech and face recognition, classification of large volumes of web data, and finance. The bottleneck is that neural network training involves iterative gradient descent and is extremely computationally intensive. In this paper we present a technique for distributed training of Ultra Large Scale Neural Networks (ULSNN) on Bunyip, a Linux-based cluster of 196 Pentium III processors. To illustrate ULSNN training we describe an experiment in which a neural network with 1.73 million adjustable parameters was trained to recognize machine-printed Japanese characters from a database containing 9 million training patterns. The training runs with a average performance of 163.3 GFlops/s (single precision). With a machine cost of \$150,913, this yields a price/performance ratio of 92.4c/MFlops/s (single precision). For comparison purposes, training using double precision and the ATLAS DGEMM produces a sustained performance of 70 MFlops/s or \$2.16 / MFlop/s (double precision).

==> Makefile <==

TEXFILE = sc2000

BIBFILE = Bib/bib

FIGURES =  figures/iter.eps figures/l1block.eps figures/emmperf.eps \
	 	figures/reduce.eps figures/genperf.eps figures/procscale.eps

OTHERS = abstract.tex intro.tex conclusion.tex hardware.tex sgemm.tex nn.tex \
         jocr.tex experiment.tex results.tex Texdefs/mathdefs.tex \
	 reduce.tex $(FIGURES)

# ########## Shouldn't need to change anything below here. ########## #

SHELL = /bin/sh

XDVI = xdvi
BIBTEX = bibtex
LATEX = latex
PDFTEX = pdflatex
DVIPS = dvips -ta4
FIG2DEV = fig2dev
LP = lpr -Pcsldp

$(TEXFILE).dvi: $(OTHERS) $(TEXFILE).bbl $(TEXFILE).tex
	$(LATEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE); 
	$(LATEX) $(TEXFILE); 
	$(LATEX) $(TEXFILE);

$(TEXFILE).pdf: $(OTHERS) $(TEXFILE).bbl $(TEXFILE).tex
	$(PDFTEX) $(TEXFILE)
	$(BIBTEX) $(TEXFILE); 
	$(PDFTEX) $(TEXFILE); 
	$(PDFTEX) $(TEXFILE);


$(PSTEXFIGS) : $(@:pstex_t=fig)
	$(FIG2DEV) -L pstex_t -p $(@:pstex_t=pstex) $(@:pstex_t=fig) $@
	$(FIG2DEV) -L pstex $(@:pstex_t=fig) $(@:pstex_t=pstex)
	fixpstex.sh $@

$(TEXFILE).bbl: $(BIBFILE).bib
	if test ! -r $(TEXFILE).aux; then \
		$(LATEX) $(TEXFILE); \
	fi
	$(BIBTEX) $(TEXFILE)

$(TEXFILE).ps: $(TEXFILE).dvi
	$(DVIPS) -o $(TEXFILE).ps $(TEXFILE).dvi

.PHONY: x tidy clean spotless print

x: $(TEXFILE).dvi
	$(XDVI) $(TEXFILE) &

tidy:
	rm -f *~ *.bak figures/*.pstex*

clean: tidy
	rm -f $(TEXFILE).aux $(TEXFILE).log $(TEXFILE).dvi \
	       $(TEXFILE).ps $(TEXFILE).bbl $(TEXFILE).blg \

spotless: clean
	rm -f $(TEXFILE).dvi $(TEXFILE).ps

print: $(TEXFILE).ps
	$(LP) $(TEXFILE).ps


==> Texdefs/bookdefs.tex <==
\input{../Texdefs/common}

%% theorem-like environments
\newtheorem{theorem}{Theorem}[chapter]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}

\newenvironment{exercises}{%
    \section{Exercises}
    % \renewcommand\theenumi{\thechapter.\@arabic\c@enumi}
    \begin{enumerate}
  }{%
    \end{enumerate}
    % \renewcommand\theenumi{\@arabic\c@enumi}
  }


==> Texdefs/mathdefs.tex <==
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\TD}{TD}
\DeclareMathOperator{\VCdim}{VCdim}
\DeclareMathOperator{\MCG}{MCG}
\DeclareMathOperator{\GPOMDP}{GPOMDP}
\DeclareMathOperator{\CONJGRAD}{CONJPOMDP}
\DeclareMathOperator{\OLPOMDP}{OLPOMDP}
\DeclareMathOperator{\REINFORCE}{REINFORCE}
\DeclareMathOperator{\MDP}{MDP}
\DeclareMathOperator{\POMDP}{POMDP}
\DeclareMathOperator{\POMDPG}{POMDPG}
\DeclareMathOperator{\GSEARCH}{GSEARCH}
\DeclareMathOperator{\REWARD}{REWARD}
\DeclareMathOperator{\VAL}{VAL}
\DeclareMathOperator{\GRAD}{GRAD}
\DeclareMathOperator{\er}{er}

\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newcommand{\td}{TD($\lambda$)\xspace}
\newcommand{\Jm}{{J^{\mu}}}
\newcommand{\Jh}{{\Hat{J}}}

\newcommand{\mcg}{{\mbox{\small$\MCG$}}}
\newcommand{\pomdpg}{{\mbox{\small$\GPOMDP$}}}
\newcommand{\conjgrad}{{\mbox{\small$\CONJGRAD$}}}
\newcommand{\olpomdp}{{\mbox{\small$\OLPOMDP$}}}
\newcommand{\reinforce}{{\mbox{\small$\REINFORCE$}}}
\newcommand{\mdp}{{\mbox{\small$\MDP$}}}
\newcommand{\mdps}{{\mbox{\small$\MDP$}}s}
\newcommand{\pomdp}{{\mbox{\small$\POMDP$}}}
\newcommand{\pomdps}{{\mbox{\small$\POMDP$}}s}
\newcommand{\gsearch}{{\mbox{\small$\GSEARCH$}}}
\newcommand{\reward}{{\mbox{\small$\REWARD$}}}
\newcommand{\val}{{\mbox{\small$\VAL$}}}
\newcommand{\grad}{{\mbox{\small$\GRAD$}}}
\newcommand{\pt}{{\tilde p}}
\newcommand{\qt}{{\tilde q}}
\newcommand{\erh}{{\hat{\er}}}
\newcommand{\etah}{{\hat{\eta}}}
\newcommand{\etat}{{\tilde{\eta}}}
\newcommand{\dhat}{{\hat{d}}}
\newcommand{\h}{{\mathbold{h}}}
\newcommand{\Pb}{{\mathbold{P}}}
\newcommand{\scPb}{{\mathbold{\scriptstyle P}}}
\newcommand{\mathbold}[1]{\mbox{\boldmath $\bf#1$}}
\newcommand{\glossaryentry}[3]{\item[#1] #2 \hfill #3}
\newcommand{\nb}{{\nabla_{\!\!\beta}}}
\renewcommand{\Box}{\square}
\renewcommand{\glossary}[2]{}
\def\addcontentsline#1#2#3{} 
\newtheorem{thm}{Theorem}
\newtheorem{exmp}{Example}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{corr}[thm]{Corollary}
\newtheorem{defn}{Definition}
\newcommand{\D}{{\cal D}}
\newcommand{\ie}{{\em i.e.\ }}
\newcommand{\etal}{{\em et.\ al.\ }}
\newcommand{\iid}{{i.i.d.\ }}
\newcommand{\norm}{{\|\cdot\|}}
\newcommand{\eg}{{\em e.g.\ }}
\newcommand{\cf}{{\em c.f.\ }}
\newcommand{\etc}{{\em etc}}
\newcommand{\comp}[2]{{#1\circ#2}}
\newcommand{\epspic}[2]{{\parbox{#1}{\epsfxsize=#1\epsfbox{#2}}}}
\renewcommand{\d}[2]{d_\nu\left(#1,#2\right)}
\newcommand{\rangel}[1]{\rangle_{#1}}
\newcommand{\E}{\mathbold{E}}
\newcommand{\Expect}{\mathbold{E}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\Hs}{{\HH_\sigma}}
\renewcommand{\H}{{\cal H}}
\newcommand{\XY}{{X\times Y}}
\newcommand{\VY}{{V\times Y}}
\newcommand{\de}{=}%%{{\,\,\,\,\overset{\text{def}}{=}\,\,\,\,}}
\renewcommand{\P}{{\cal P}}
\newcommand{\PP}{{\cal P}}
\newcommand{\Zm}{{\(X\timesY\)^m}}
\newcommand{\Zn}{{\(X\timesY\)^n}}
\newcommand{\Zmn}{{\(X\timesY\)^{(m,n)}}}
\newcommand{\Znm}{{\(X\timesY\)^{(n,m)}}}
\newcommand{\Ztmn}{{\(X\timesY\)^{(2m,n)}}}
\newcommand{\Gtmn}{{\Gamma_{(2m,n)}}}
\newcommand{\zmn}{{z^{(m,n)}}}
\newcommand{\znm}{{z^{(n,m)}}}
\newcommand{\z}{{\mathbold{z}}}
\newcommand{\f}{{\mathbold{f}}}
\newcommand{\g}{{\bf g}}
\newcommand{\w}{{\bf w}}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
\newcommand{\B}{{\cal B}}
\newcommand{\calB}{{\cal B}}
\newcommand{\Q}{{\cal Q}}
\newcommand{\Pm}{{P^m}}
\newcommand{\zb}{{\bold{z}}}
\newcommand{\zbh}{{\hat{\zb}}}
\newcommand{\zbv}{{\smash[b]{\vec{\zb}}}}
\newcommand{\zbvh}{\zbv} %%{\smash[b]{\hat{\vec{\zb}}}}}
\newcommand{\zh}{{\hat z}}
\newcommand{\xh}{{\hat x}}
\newcommand{\sh}{{\hat s}}
\newcommand{\Xhat}{{\hat X}}
\newcommand{\Shat}{{\hat S}}
\newcommand{\Ehat}{{\hat E}}
\newcommand{\qhat}{{\hat q}}
\newcommand{\yh}{{\hat y}}
\newcommand{\Phat}{{\hat \P}}
\newcommand{\Phihat}{{\hat \Phi}}
\newcommand{\Psihat}{{\hat \Psi}}
\newcommand{\Jt}{{\tilde{J}}}
\newcommand{\Vt}{{\tilde{V}}}
\newcommand{\Js}{{J^*}}
\newcommand{\nablat}{\nabla}
\newcommand{\Ph}{{\hat P}}
\newcommand{\zs}{{\z_\sigma}}
\newcommand{\zsw}{{\z_\sigma(1)}}
\newcommand{\zst}{{\z_\sigma(2)}}
\newcommand{\zsij}{{\z_{\sigma(ij)}}}
\newcommand{\fhat}{{\hat f}}
\newcommand{\ghat}{{\hat g}}
\newcommand{\Fhat}{{\hat \F}}
\newcommand{\rhat}{{\hat \rho}}
\newcommand{\Eh}{{\hat E}}
\newcommand{\bw}{{\bold{w}}}
\newcommand{\be}{\begin{equation*}}
\newcommand{\ee}{$$}
\newcommand{\ep}{{\varepsilon}}
\newcommand{\Z}{{\cal Z}}
\newcommand{\A}{{\cal A}}
\newcommand{\C}{{\cal C}}
\newcommand{\N}{{\cal N}}
\newcommand{\Nco}{{\N_\co}}
\newcommand{\M}{{\cal M}}
\newcommand{\F}{{\cal F}}
\newcommand{\G}{{\cal G}}
\newcommand{\T}{{\mathbb T}}
\newcommand{\calT}{{\cal T}}
\newcommand{\U}{{\cal U}}
\newcommand{\calU}{{\cal U}}
\newcommand{\V}{{\cal V}}
\newcommand{\Y}{{\cal Y}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calS}{{\cal S}}
\newcommand{\Ch}{{\hat \C}}
\newcommand{\rhol}{\rho_{\!_l}}
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
%PLB YUCK YUCK YUCK
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\newcommand{\Pv}{{\vec{P}}}
\newcommand{\xb}{{\bold{x}}}
\newcommand{\yb}{{\bold{y}}}
\newcommand{\wb}{{\bold{w}}}
\newcommand{\Deltabar}{{\overline\Delta}}
\newcommand{\Fbar}{{\overline\F}}
\newcommand{\Gbar}{{\overline\G}}
\newcommand{\Pbar}{{\bar{P}}}
\renewcommand{\hbar}{{\overline h}}
\newcommand{\dbar}{{d^*}}
\newcommand{\rbar}{{\bar{r}}}
\newcommand{\Jbar}{{\bar{J}}}
\newcommand{\co}{{\text{\rm co}}}
\newcommand{\jon}{{\text{\rm jon}}}
\newcommand{\cdm}{{d_{\text{\rm CDM}}}}
\newcommand{\cdmhat}{{\hat{d}_{\text{\rm CDM}}}}
\newcommand{\cdmhathat}{{\tilde{d}_{\text{\rm CDM}}}}
\newcommand{\lin}{{\text{\rm lin}}}
\newcommand{\sign}{{\text{\rm sign}}}
\newcommand{\IID}{{\text{\rm IID}}}
\newcommand{\OTS}{{\text{\rm OTS}}}
\newcommand{\CDM}{{\text{\rm CDM}}}
\newcommand{\VC}{{\text{\rm VC}}}
\newcommand{\cobar}[1]{{\overline{\text{\rm co}\(#1\)}}}
\newcommand{\linbar}[1]{{\overline{\text{\rm lin}\(#1\)}}}
\newcommand{\Cbar}{{{\cal C}^*}}
\newcommand{\fbar}{{\bar f}}
\newcommand{\lbar}{{\bar l}}
\newcommand{\pibar}{{\bar \pi}}
\newcommand{\zv}{{\vec{z}}}
\newcommand{\gv}{{\vec{g}}}
\newcommand{\fv}{{\mathbold{f}}}
\newcommand{\lv}{{\vec l}}
\newcommand{\hv}{{\vec h}}
\newcommand{\xv}{{\mathbold{x}}}
\newcommand{\yv}{{\vec y}}
\newcommand{\wv}{{\mathbold{w}}}
\newcommand{\vv}{{\vec v}}
\newcommand{\av}{{\vec a}}
\newcommand{\Xv}{{\vec X}}
\newcommand{\pr}[3]{{{#1}_1#2\dots#2{#1}_{#3}}}
\newcommand{\iton}{{1\leq i\leq n}}
\newcommand{\prd}[4]{{{#1}_{#2}#3\dots#3{#1}_{#4}}}
\newcommand{\R}{{\mathbb R}}
\renewcommand{\Re}{{\R}}
\newcommand{\Rn}{{\R^n}}
\newcommand{\Rpm}{{(\mathbb R^+)^{2m}}}
\newcommand{\Rptm}{{(\mathbb R^+)^{(2m,n)}}}
\newcommand{\dl}{{\mbox{\boldmath$d_{L^1}$}}}
\newcommand{\dimp}{{\mbox{dimp}}}
\newcommand{\argmin}{{\mbox{argmin}}}
\newcommand{\plus}{{\mbox{plus}}}
\newcommand{\minus}{{\mbox{minus}}}
\newcommand{\DKL}{{\mbox{DKL}}}
\newcommand{\WKS}{{\mbox{WKS}}}
\newcommand{\PKS}{{\mbox{PKS}}}
\newcommand{\ch}{{\large \chi}}
\newcommand{\SZ}{{\cal S}_Z}
\newcommand{\SP}{{\cal S}_\P}
\newcommand{\Tbar}{{\overline T}}
\newcommand{\Sbar}{{\overline S}}
\newcommand{\Xbar}{{\overline X}}
\newcommand{\Hbar}{{\overline \H}}
\newcommand{\bool}{{\{\pm 1\}}}
\newcommand{\zm}{{z^m}}
%\newcommand{\Hns}{{\[\HH^n\]_\sigma}}
%\newcommand{\Hsn}{{\[\HH_\sigma\]^n}}
\newcommand{\XVA}{X\stackrel{\F}{\rightarrow}V\stackrel{\G}{\rightarrow}A}
\newcommand{\XfVGY}{X\stackrel{f}{\rightarrow}V\stackrel{\G}{\rightarrow}Y}










